Singularities on the boundary of the stability domain near 1:1 resonance

We study the linear differential equation x' = Lx in 1:1 resonance. That is, x in R^4 and L is a 4 by 4 matrix with a semi-simple double pair of imaginary eigenvalues (ib,-ib,ib,-ib). We wish to find all perturbations of this linear system such that the perturbed system is stable. Since linear differential equations are in one to one correspondence with linear maps we translate this problem to gl(4,R). In this setting our aim is to determine the stability domain and the singularities of its boundary. The dimension of gl(4,R) is 16, therefore we first reduce the dimension as far as possible. Here we use a versal unfolding of L ie a transverse section of the orbit of L under the adjoint action of Gl(4,R). Repeating a similar procedure in the versal unfolding we are able to reduce the dimension to 4. A 3-sphere in this 4-dimensional space contains all information about the neighborhood of L in gl(4,R). In this 3-sphere the boundary of the stability domain is a surface with singularities: transverse self-intersections, Whitney umbrellas and an intersection of self-intersections where the surface has a self-tangency.

==> Makefile <==
# set latexfile to the name of the main file without the .tex
LATEXFILE = stabrega
# put the names of figure files here.
FIGURES =\
	conoid.eps\
	conoids.eps\
	domain.ps\
	eigcfgs.ps\
	incid.ps\
	phipsi.ps\
	saddles.eps\
	skelet1.ps\
	skelet2.ps\
	transorb.ps\
	whitney.eps
TEX = latex
DATE = `date +%Y%b%d`

# reruns latex if needed. to get rid of this capability, delete the
# three lines after the rule. 
# idea from http://ctan.unsw.edu.au/help/uk-tex-faq/Makefile
$(LATEXFILE).dvi : $(FIGURES) $(LATEXFILE).tex
	while ($(TEX) $(LATEXFILE) ; \
	grep -q "Rerun to get cross" $(LATEXFILE).log ) do true ; \
	done

$(LATEXFILE).pdf : $(LATEXFILE).ps
	ps2pdf $(LATEXFILE).ps $(LATEXFILE).pdf

pdf : $(LATEXFILE).pdf

$(LATEXFILE).ps : $(FIGURES) $(LATEXFILE).dvi
	dvips $(LATEXFILE)

ps : $(LATEXFILE).ps

clean :
	rm $(LATEXFILE).aux $(LATEXFILE).dvi $(LATEXFILE).log $(LATEXFILE).ps $(LATEXFILE).toc *~

$(LATEXFILE).tar : $(FIGURES) $(LATEXFILE).tex
	tar -cvf $(LATEXFILE)-$(DATE).tar $(FIGURES) $(LATEXFILE).tex $(LATEXFILE).pdf Makefile

tarball: $(LATEXFILE).tar

